EOL: Transductive Few-Shot Open-Set Recognition by Enhancing Outlier Logits

In Few-Shot Learning (FSL), models are trained to recognise unseen objects from a query set, given a few labelled examples from a support set. In standard FSL, models are evaluated on query instances sampled from the same class distribution of the support set. In this work, we explore the more nuanced and practical challenge of Open-Set Few-Shot Recognition (OSFSL). Unlike standard FSL, OSFSL incorporates unknown classes into the query set, thereby requiring the model not only to classify known classes but also to identify outliers. Building on the groundwork laid by previous studies, we define a novel transductive inference technique that leverages the InfoMax principle to exploit the unlabelled query set. We called our approach the Enhanced Outlier Logit (EOL) method. EOL refines class prototype representations through model calibration, effectively balancing the inlier-outlier ratio. This calibration enhances pseudo-label accuracy for the query set and improves the optimisation objective within the transductive inference process. We provide a comprehensive empirical evaluation demonstrating that EOL consistently surpasses traditional methods, recording performance improvements ranging from approximately $+1.3%$ to $+6.3%$ across a variety of classification and outlier detection metrics and benchmarks, even in the presence of inlier-outlier imbalance.

==> chapter_openset/figures/ablation_lambda.tex <==
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.24\linewidth]{chapter4/figures/incrqueries_acc.pdf}
%     \includegraphics[width=0.24\linewidth]{chapter4/figures/incrqueries_rocauc.pdf}
%     \includegraphics[width=0.24\linewidth]{chapter4/figures/incrqueries_aupr.pdf}
%     \includegraphics[width=0.24\linewidth]{chapter4/figures/incrqueries_prec_at_90.pdf}
%     \caption{Increasing the number of queries per class}
%     \label{ch:openset:fig:incrqueries}
% \end{figure*}

==> chapter_openset/figures/ablation_proto.tex <==
\begin{figure*}[tbhp]
    \centering
    \includegraphics[width=0.33\linewidth]{chapter4/figures/oodproto_ablation_ALTIMProved_val_acc.pdf}
    \includegraphics[width=0.33\linewidth]{chapter4/figures/oodproto_ablation_ALTIMProved_val_rocauc.pdf}
    \includegraphics[width=0.33\linewidth]{chapter4/figures/oodproto_ablation_ALTIMProved_val_cum.pdf}
    \caption{Varying the number of outlier prototypes and Dirichlet $\alpha_{\text{proto}}$ parameter. The figure shows that method is largely insensitive to the exact parameter choice.}
    \label{ch:openset:fig:incrqueries}
\end{figure*}

==> chapter_openset/figures/incroodway.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{chapter4/figures/way5_incroodway_rocauc.pdf}
    \caption{Increasing the number of outlier classes, $N_{\text{out}}$}
    \label{ch:openset:fig:my_label}
\end{figure}

==> chapter_openset/figures/incrqueries.tex <==
\begin{figure*}[thbp]
    \centering
    \includegraphics[width=0.49\linewidth]{chapter4/figures/incrqueries_acc.pdf}
    \includegraphics[width=0.49\linewidth]{chapter4/figures/incrqueries_rocauc.pdf}
    \includegraphics[width=0.49\linewidth]{chapter4/figures/incrqueries_aupr.pdf}
    \includegraphics[width=0.49\linewidth]{chapter4/figures/incrqueries_prec_at_90.pdf}
    \caption{Increasing the number of queries per class}
    \label{ch:openset:fig:incrqueries}
\end{figure*}

==> chapter_openset/tables/main_results.tex <==
\begin{table}[t]
\centering
\small
\caption{\textbf{Open-Set Few-Shot Learning Task.} * Indicates results taken from \cite{}. }
\label{ch:openset:tab:benchmark_results_mini}
\renewcommand{\arraystretch}{1.4}
\centering
\begin{tabular}{c|l|cccc}
                %  &     &  \multicolumn{4}{c}{mini-ImageNet} \\
                 & & Acc. & AUROC & AUPR & Prec@90 \\ 
                    \midrule
    \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{1-shot}}} & OSTIM*          & \rcell{69.23}{0.72} & \rcell{74.3}{0.79} & \rcell{75.01}{0.69} & \rcell{59.93}{0.47} \\
    &  OSTIM           & \rcell{68.86}{0.68}	&	\rcell{74.76}{0.60}	&	\rcell{75.31}{0.63}	&	\rcell{60.21}{0.48} \\
    % OSTIM (no loop) &  &  &  &  \\
    % \midrule
     & \rowcolor{lightgray!25} OSTIMOP  & \rcell{70.19}{0.74}	&\rcell{76.24}{0.66}	&\rcell{75.84}{0.68}	&\rcell{61.97}{0.60}  \\
    % OSTIMOP (no loop)  &  &  &  &  \\
    % \bottomrule
                    \midrule
   \parbox[t]{1mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{5-shot}}} & OSTIM*    & \rcell{82.79}{0.44} & \rcell{83.80}{0.73} & \rcell{84.30}{0.61} & \rcell{67.46}{0.56} \\
     &  OSTIM           & \rcell{82.22}{0.43}	&\rcell{83.81}{0.43}	&\rcell{84.10}{0.45}	&\rcell{67.62}{0.59} \\
    % OSTIM (no loop) &  &  &  &  \\
    % \midrule
     & \rowcolor{lightgray!25} OSTIMOP  & \rcell{\textbf{83.72}}{\textbf{0.42}}	& \rcellbest{85.82}{0.44}	&\rcell{85.86}{0.45}	&\rcell{70.46}{0.67}  \\
    % OSTIMOP (no loop)  &  &  &  &  \\
    \bottomrule
\end{tabular}
\end{table}

==> chapter_openset/tables/mini_results.tex <==
\begin{table*}[t]
\centering
\small
\caption{\textbf{Standard Benchmarking}. \todo{Change:} Evaluating different families of methods on the FSOSR problem, on the popular \textit{mini}-ImageNet, using a ResNet-12. For each column, a light-gray standard deviation is indicated, corresponding to the maximum deviation observed across methods for that metric. Best methods are shown in bold. Results for PEELER$^\star$ are reported from \cite{jeong2021few}. The same table for \textit{tiered}-ImageNet is available in Appendix, along with the details about the presented metrics.}
% \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        \multicolumn{10}{c}{\textbf{\textit{mini}-ImageNet}} \vspace{0.5em}\\
        \toprule
        \multirow{3}{*}{Strategy} & \multirow{3}{*}{Method} & \multicolumn{4}{c}{1-shot} & \multicolumn{4}{c}{5-shot} \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-10}
        & & Acc & AUROC & AUPR & Prec@0.9 & Acc & AUROC & AUPR & Prec@0.9 \\
        & & \std{0.72} & \std{0.79} & \std{0.69} & \std{0.47} & \std{0.44} & \std{0.73} & \std{0.61} & \std{0.56} \\
        \midrule
        \multirow{6}{*}{OOD detection} & \knn \cite{knn_detector} & - & 70.28 & 69.78 & 58.01 & - & 76.56 & 76.75 & 61.58 \\
                                      & IForest \cite{iforest_detector} & - & 56.10 & 55.54 & 52.34 & - & 63.46 & 62.21 & 55.09 \\
                                      & OCVSM \cite{ocsvm_detector} & - & 69.25 & 69.15 & 57.35 & - & 69.25 & 66.38 & 59.43 \\
                                      & PCA \cite{pca_detector} & - & 67.14 & 66.33 & 56.78 & - & 75.31 & 75.59 & 60.54 \\
                                      & COPOD \cite{copod_detector} & - & 50.45 & 51.76 & 50.86 & - & 52.70 & 53.6 & 51.47 \\
                                      & HBOS  & - & 58.25 & 57.39 & 53.32 & - & 61.62 & 60.64 & 54.47 \\

        \toprule
        \multirow{3}{*}{Inductive classifiers} & SimpleShot \cite{wang2019simpleshot} & 65.93 & 64.44 & 63.27 & 55.29 & 81.73 & 70.92 & 70.36 & 58.13 \\
                                              & Baseline ++ \cite{chen19} &  65.91 & 64.61 & 63.32 & 55.41 & 81.87 & 66.65 & 65.74 & 56.53 \\
                                              & FEAT \cite{ye2020few} & 67.28 & 52.25 & 54.28 & 50.0 & 81.89 & 53.25 & 56.36 & 50.0 \\
        \midrule
        \multirow{4}{*}{Inductive Open-Set} & PEELER$^\star$ \cite{liu2020peeler} & 65.86 & 60.57 & - & - & 80.61 & 67.35 & - & - \\
                                            & SnatcherF \cite{jeong2021few}  & 67.28 & 69.26 & 68.98 & 57.57 & 81.89 & 76.87 & 77.35 & 62.09  \\
                                            & OpenMax \cite{bendale2016towards} & 65.93 & 70.86 & 70.34 & 58.30 &  82.37 & 77.34 & 77.62 & 62.14  \\
                                            & PROSER \cite{zhou2021learning} & 64.89 & 68.63 & 68.42 & 57.19 & 80.09 & 75.0 & 75.64 & 60.18 \\
        \toprule
        \multirow{5}{*}{Transductive classifiers} & LaplacianShot \cite{ziko2020laplacian} & {70.99} & 51.88 & 53.59 &     51.66 &  {82.88} & 57.17 & 57.88 &     52.66   \\
                                                  & BDCSPN \cite{liu2020prototype} &  69.88 & 56.98 &     57.87 &     52.12 & {82.50}  & 61.52 &     62.29 &     53.44 \\
                                                  & TIM-GD \cite{boudiaf2020transductive} & 67.78 & 61.94 &     60.71 &     54.48 & {82.51} & 67.29 &     66.05 &     56.87 \\
                                                  & PT-MAP \cite{hu2021leveraging} & 66.29 & 58.66 &    58.32 &     53.44 & 77.72 & 63.22 &     62.89 &     54.77 \\
                                                  & LR-ICI \cite{wang2020instance} & 69.34 & 46.10	& 49.24 & 50.02 & 81.46 & 45.97 & 49.84 & 49.91 \\
        % \rowcolor{lightsalmon!25} Transductive Open-Set & \OSTIM (ours) & 69.23 & {73.08} & {74.32} &  \textbf{58.96} &  {82.79} & {83.80}  & {84.30}  &  \textbf{67.46} \\
        \midrule
        \multirow{3}{*}{Transductive Open-Set} & \OSTIM \cite{boudiaf2022ostimop} & 69.23 & 74.3 & 75.01 &  59.93 & 82.79 & 83.80  & 84.30  &  67.46 \\
        % \midrule
         & \rowcolor{lightsalmon!25} OSTIMOP (ours) & \textbf{70.95} & \textbf{75.70} & \textbf{76.06} &  \textbf{60.94} &  \textbf{83.39} & \textbf{86.15}  & \textbf{85.97}  &  \textbf{71.31} \\
        % \bottomrule
        & \rowcolor{lightgray!25} \emph{improvement} & \emph{+1.72} & \emph{+1.40} & \emph{+1.05} & \emph{+1.01} & \emph{+0.60} & \emph{+2.35} & \emph{+1.67} & \emph{+3.85} \\
        \bottomrule
    \end{tabular}
% } 
\label{ch:openset:tab:benchmark_results_mini}
\end{table*}

==> chapter_openset/tables/osem_results_append.tex <==
% \begin{table*}[t]
%     \centering
%     \small
%     \caption[Standard Balanced Open Set Few-Shot Task]{\textbf{Standard Balanced Open Set Few-Shot Task}. Evaluating different families of methods on the FSOSR problem on \textit{mini}-ImageNet using a ResNet-12. Best methods are shown in bold. Results marked with $^\star$ are reported from their original paper.}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        & & \multicolumn{8}{c}{\textbf{ \textit{mini}-ImageNet}} \vspace{0.5em}\\
        \toprule
        \multirow{3}{*}{Strategy} & \multirow{3}{*}{Method} & \multicolumn{4}{c}{1-shot} & \multicolumn{4}{c}{5-shot} \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-10}
        & & Acc & AUROC & AUPR & Prec@0.9 & Acc & AUROC & AUPR & Prec@0.9 \\
        & & \std{0.72} & \std{0.79} & \std{0.69} & \std{0.47} & \std{0.44} & \std{0.73} & \std{0.61} & \std{0.56} \\
        \midrule
        \multirow{6}{*}{\specialcell{OOD\\detection}} & \knn \cite{knn_detector} &      -     &         70.86 &       70.43 &             58.23 &      -     &         76.22 &       76.36 &             61.48  \\
                                        & IForest \cite{iforest_detector}  &      -     &         55.59 &       55.24 &             52.18 &      -     &         62.80 &       61.62 &             54.77  \\
                                        & OCVSM \cite{ocsvm_detector}  &      -     &         69.67 &       69.71 &             57.35 &      -     &         68.49 &       65.60 &             59.24  \\
                                        & PCA \cite{pca_detector}  &      -     &         67.23 &       66.50 &             56.67 &      -     &         75.24 &       75.53 &             60.73  \\
                                        & COPOD \cite{copod_detector}  &      -     &         50.60 &       51.85 &             50.92 &      -     &         51.63 &       52.65 &             51.31  \\
                                        & HBOS                 &      -     &         58.26 &       57.41 &             53.06 &      -     &         61.11 &       60.18 &             54.30  \\

        \toprule
        \multirow{3}{*}{\specialcell{Inductive\\classifiers}} & SimpleShot \cite{wang2019simpleshot} &      65.90 &         64.99 &       63.78 &             55.77 &      81.72 &         70.61 &       70.06 &             57.91 \\
                                                & Baseline ++ \cite{chen2019closerfewshot}&      65.81 &         65.15 &       63.85 &             55.87 &      81.86 &         66.37 &       65.58 &             56.33 \\
                                                & FEAT  \cite{ye2020few}  &      67.23 &         52.45 &       54.44 &             50.00 &      82.00 &         53.25 &       56.48 &             50.00 \\

        \midrule
        \multirow{5}{*}{\specialcell{Inductive\\Open-Set}} & PEELER$^\star$ \cite{liu2020peeler} & 65.86 & 60.57 & - & - & 80.61 & 67.35 & - & - \\
                                            & TANE-G$^\star$ \cite{huang2022task} & 68.11 & 72.41 & - & - & 83.12 & 79.85 & - & - \\
                                            & SnatcherF \cite{jeong2021snatcher} &      67.23 &         70.10 &       69.74 &             58.02 &      82.00 &         76.57 &       76.97 &             61.64 \\
                                            & OpenMax \cite{bendale2016towards} &      65.90 &         71.34 &       70.86 &             58.67 &      82.23 &         77.42 &       77.63 &             62.35 \\
                                            & PROSER \cite{zhou2021learning} &      65.00 &         68.93 &       68.84 &             57.03 &      80.08 &         74.98 &       75.58 &             60.11 \\

        \toprule
        \multirow{5}{*}{\specialcell{Transductive\\classifiers}} & LaplacianShot \cite{ziko2020laplacian} & 70.59 &         53.13 &       54.59 &             52.06 &  82.94 &         57.17 &       57.90 &             52.56 \\
                                                    & BDCSPN \cite{liu2020prototype} &      69.35 &         57.95 &       58.58 &             52.71 &    82.66 &         61.27 &       62.17 &             53.26 \\
                                                    & TIM-GD \cite{boudiaf2020transductive}  &      67.53 &         62.46 &       61.05 &             54.83 &      82.49 &         67.19 &       66.15 &             56.70 \\
                                                    & PT-MAP \cite{hu2021leveraging}  &      66.32 &         59.05 &       58.67 &             53.74 &      78.12 &         62.78 &       62.48 &             54.67 \\
                                                    & LR-ICI \cite{wang2020instance}  &      68.24 &         49.96 &       51.61 &             50.45 &      81.77 &         51.82 &       53.49 &             50.80 \\

        \midrule
        \multirow{2}{*}{\specialcell{Transductive\\Open-Set}} & OSLO* \cite{boudiaf2023osem}  &  \textbf{71.73} &        74.92 &     74.61 &       60.95  &     \textbf{83.40} &   82.59 &      82.34 &       66.98 \\
                                                & OSTIM* \cite{boudiaf2022ostim}  & 69.23 &      74.30 &     75.01 &       59.93  &     82.79 &   83.88 &      84.30 &       67.46 \\
                                                \rowcolor{green!8} & OSTIM (ITER=0)  &  66.40  &    74.88    &   73.92   &   61.34    &     81.65 &   83.61 &      83.38 &    67.90 \\
                                                \rowcolor{red!8} & \ourmethod (ours)  &  69.63  &    \textbf{77.00}    &    \textbf{76.34}   &     \textbf{63.20}    &     83.31 &   \textbf{86.61} &      \textbf{86.11} &       \textbf{72.25} \\
    \end{tabular}
}
% \end{table*}

==> chapter_openset/tables/ours_disect_param2adapt.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption[Table showing the deeper analysis of algorithms.]{Table showing the performance of the algorithms while leaving out some components from the algorithm, such as the scalling ($a$) and shifting ($b$) of inlier logits parameters and the prototype ($c$). When only the prototypes are adapted during infererence, the algorithm becomes more similar to OSTIM\cite{boudiaf2022ostim} but with more appropiately balanced inlier and outlier samples. On the other hand, fine-tuning the `abc' parameters (equivalent to \ourmethod) results in better algorithm all together.}\label{ch:openset:tab:ours_disect_param2adapt}
    \begin{tabular}{lrrrr}
        \toprule
        {} &  Acc. &  AUROC &  AUPR &  Prec.@90 \\
        % params2adapt &       &        &       &           \\
        \midrule
        a,b,c        & 83.21 &  86.62 & 86.12 &     72.26 \\
        c            & 82.09 &  84.95 & 84.91 &     69.12 \\
        a,b          & 82.37 &  84.68 & 84.15 &     69.26 \\
        \bottomrule
    \end{tabular}
\end{table*}


==> chapter_openset/tables/query1.tex <==
{
\newcommand{\osrcolor}{\rowcolor{blue!8}}
\newcommand{\fslcolor}{\rowcolor{green!8}}
\newcommand{\fsosrcolor}{\rowcolor{orange!8}}
\newcommand{\tfslcolor}{\rowcolor{red!8}}
\newcommand{\tfsosrcolor}{\rowcolor{lightgray!10}}
\newcommand{\ourscolor}{\tfsosrcolor}
\newcommand{\citeignore}[1]{ }


\begin{table}[htbp]
\caption{\textbf{Open-Set Few-Shot Learning Task with evaluated at 1-query sample at a time.} \textcolor{blue!50}{Blue} background indicates classical OSR methods, \textcolor{green!50}{green} is for inductive FSL methods, \textcolor{orange!50}{orange} is for inductive FSOSR methods, \textcolor{red!50}{red} indicates transductive FSL algorithms, and \textcolor{lightgray!70}{gray} is for transductive FSOSR algorithms. }
\label{ch:openset:tab:query1}
\centering
\renewcommand{\arraystretch}{1.4}
\scalebox{0.87}{
\begin{tabular}{ll|cccc}
\toprule
       &                &                        Acc. &                       AUROC &                        AUPR &                     Prec@90 \\
% {} & Method &                             &                             &                             &                             \\
\midrule
\sidecell{15}{1-shot} & \osrcolor \knn \citeignore{knn_detector} &                  \emptycell &     \rcellbest{71.35}{0.91} &     \rcellbest{71.73}{0.97} &     \rcellbest{61.13}{0.88} \\
       & \osrcolor OCVSM \citeignore{ocsvm_detector} &                  \emptycell &         \rcell{69.91}{0.90} &  \rcellsndbest{71.05}{0.99} &  \rcellsndbest{60.58}{0.87} \\
       & \osrcolor PCA \citeignore{pca_detector} &                  \emptycell &         \rcell{67.22}{0.90} &         \rcell{67.76}{0.99} &         \rcell{58.71}{0.83} \\
       & \osrcolor HBOS &                  \emptycell &         \rcell{55.17}{0.85} &         \rcell{56.59}{0.92} &         \rcell{53.79}{0.67} \\
       & \fslcolor SimpleShot \citeignore{wang2019simpleshot} &  \rcellsndbest{65.52}{1.00} &         \rcell{64.16}{0.88} &         \rcell{64.52}{0.97} &         \rcell{57.34}{0.74} \\
       & \fslcolor Baseline ++ \citeignore{Chen19} &  \rcellsndbest{65.47}{1.00} &         \rcell{64.55}{0.87} &         \rcell{64.59}{0.96} &         \rcell{57.56}{0.75} \\
       & \fslcolor FEAT \citeignore{ye2020few} &  \rcellsndbest{65.37}{1.02} &         \rcell{62.14}{0.91} &         \rcell{62.63}{0.96} &         \rcell{56.56}{0.74} \\
       & \fsosrcolor SnatcherF \citeignore{jeong2021few} &     \rcellbest{65.74}{1.02} &         \rcell{69.21}{0.89} &         \rcell{69.30}{0.99} &         \rcell{59.99}{0.81} \\
       & \fsosrcolor OpenMax \citeignore{bendale2016towards} &  \rcellsndbest{65.52}{1.00} &  \rcellsndbest{70.68}{0.90} &         \rcell{70.64}{1.01} &  \rcellsndbest{60.84}{0.88} \\
       & \fsosrcolor PROSER \citeignore{zhou2021learning} &  \rcellsndbest{64.87}{1.02} &         \rcell{31.65}{0.92} &         \rcell{41.82}{0.78} &         \rcell{49.29}{0.62} \\
       & \tfslcolor LaplacianShot \citeignore{ziko2020laplacian} &         \rcell{64.03}{1.03} &         \rcell{61.10}{0.93} &         \rcell{61.25}{1.00} &         \rcell{56.73}{0.73} \\
       & \tfslcolor BDCSPN \citeignore{liu2020prototype} &         \rcell{63.78}{1.02} &         \rcell{61.05}{0.93} &         \rcell{61.03}{0.99} &         \rcell{56.73}{0.72} \\
       & \tfslcolor TIM-GD \citeignore{boudiaf2020transductive} &         \rcell{63.97}{1.03} &         \rcell{59.26}{0.89} &         \rcell{59.80}{0.96} &         \rcell{55.85}{0.70} \\
       & \tfslcolor PT-MAP \citeignore{hu2021leveraging} &         \rcell{58.70}{1.05} &         \rcell{57.17}{0.91} &         \rcell{57.83}{0.96} &         \rcell{54.89}{0.72} \\
       & \tfsosrcolor OSTIM \citeignore{boudiaf2022ostim} &         \rcell{63.97}{1.00} &         \rcell{66.30}{0.85} &         \rcell{65.68}{0.99} &         \rcell{58.46}{0.79} \\
       & \tfsosrcolor EOL (ours) &         \rcell{63.33}{1.00} &         \rcell{67.14}{0.83} &         \rcell{67.66}{0.97} &         \rcell{59.19}{0.78} \\
\midrule
\sidecell{17}{5-shot} & \osrcolor \knn \citeignore{knn_detector} &                  \emptycell &         \rcell{76.96}{0.80} &  \rcellsndbest{77.41}{0.90} &  \rcellsndbest{65.00}{0.94} \\
       & \osrcolor OCVSM \citeignore{ocsvm_detector} &                  \emptycell &         \rcell{75.57}{0.80} &  \rcellsndbest{77.03}{0.89} &         \rcell{63.99}{0.92} \\
       & \osrcolor PCA \citeignore{pca_detector} &                  \emptycell &         \rcell{75.72}{0.81} &         \rcell{76.22}{0.92} &         \rcell{63.70}{0.88} \\
       % & \osrcolor COPOD \citeignore{copod_detector} &                  \emptycell &         \rcell{63.41}{0.91} &         \rcell{63.26}{1.01} &         \rcell{57.59}{0.78} \\
       & \osrcolor HBOS &                  \emptycell &         \rcell{61.56}{0.92} &         \rcell{62.03}{1.00} &         \rcell{56.40}{0.77} \\
       & \fslcolor SimpleShot \citeignore{wang2019simpleshot} &  \rcellsndbest{81.63}{0.78} &         \rcell{71.37}{0.84} &         \rcell{71.10}{0.94} &         \rcell{61.39}{0.87} \\
       & \fslcolor Baseline ++ \citeignore{Chen19} &  \rcellsndbest{81.56}{0.78} &         \rcell{70.65}{0.81} &         \rcell{69.99}{0.94} &         \rcell{61.15}{0.84} \\
       & \fslcolor FEAT \citeignore{ye2020few} &         \rcell{81.20}{0.78} &         \rcell{67.88}{0.93} &         \rcell{68.03}{1.01} &         \rcell{59.22}{0.85} \\
       & \fsosrcolor SnatcherF \citeignore{jeong2021few} &  \rcellsndbest{81.43}{0.78} &     \rcellbest{77.77}{0.80} &  \rcellsndbest{77.74}{0.90} &     \rcellbest{65.70}{0.93} \\
       & \fsosrcolor OpenMax \citeignore{bendale2016towards} &     \rcellbest{82.11}{0.78} &  \rcellsndbest{77.58}{0.80} &     \rcellbest{77.81}{0.89} &  \rcellsndbest{65.51}{0.92} \\
       & \fsosrcolor PROSER \citeignore{zhou2021learning} &  \rcellsndbest{81.39}{0.77} &         \rcell{63.59}{0.84} &         \rcell{63.60}{0.96} &         \rcell{57.77}{0.75} \\
       & \tfslcolor LaplacianShot \citeignore{ziko2020laplacian} &  \rcellsndbest{81.57}{0.78} &         \rcell{70.98}{0.83} &         \rcell{69.29}{0.97} &         \rcell{62.02}{0.86} \\
       & \tfslcolor BDCSPN \citeignore{liu2020prototype} &         \rcell{80.97}{0.78} &         \rcell{69.32}{0.89} &         \rcell{68.02}{1.00} &         \rcell{61.37}{0.85} \\
       & \tfslcolor TIM-GD \citeignore{boudiaf2020transductive} &         \rcell{81.17}{0.79} &         \rcell{65.90}{0.87} &         \rcell{65.02}{0.98} &         \rcell{59.15}{0.78} \\
       & \tfslcolor PT-MAP \citeignore{hu2021leveraging} &         \rcell{81.31}{0.77} &         \rcell{67.42}{0.87} &         \rcell{66.93}{0.98} &         \rcell{59.41}{0.83} \\
       & \tfsosrcolor OSTIM \citeignore{boudiaf2022ostim} &         \rcell{81.05}{0.80} &         \rcell{74.07}{0.79} &         \rcell{72.70}{0.94} &         \rcell{63.82}{0.87} \\
       & \tfsosrcolor EOL (ours) &         \rcell{80.95}{0.77} &         \rcell{74.24}{0.78} &         \rcell{73.06}{0.93} &         \rcell{63.97}{0.85} \\
\bottomrule
\end{tabular}
}
\end{table}

}

==> chapter_openset/tables/shot1shot5_stacked.tex <==
{
\newcommand{\osrcolor}{\rowcolor{blue!8}}
\newcommand{\fslcolor}{\rowcolor{green!8}}
\newcommand{\fsosrcolor}{\rowcolor{orange!8}}
\newcommand{\tfslcolor}{\rowcolor{red!8}}
\newcommand{\tfsosrcolor}{\rowcolor{lightgray!10}}
\newcommand{\ourscolor}{\tfsosrcolor}
\newcommand{\citeignore}[1]{ }

\begin{table}[htbp]
\caption{\textbf{Open-Set Few-Shot Learning Task.} \textcolor{blue!50}{Blue} background indicates classical OSR methods, \textcolor{green!50}{green} is for inductive FSL methods, \textcolor{orange!50}{orange} is for inductive FSOSR methods, \textcolor{red!50}{red} indicates transductive FSL algorithms, and \textcolor{lightgray!70}{gray} is for transductive FSOSR algorithms. }
\label{ch:openset:tab:benchmark_results_mini}
\centering
\renewcommand{\arraystretch}{1.4}
\scalebox{0.87}{
\begin{tabular}{ll|cccc}
\toprule
       &                &                        Acc. &                    AUROC &                     AUPR &                  Prec@90 \\
% {} & method &                             &                          &                          &                          \\
\midrule
\sidecell{17}{1-shot} & \osrcolor \knn \citeignore{knn_detector} &                  \emptycell &      \rcell{71.19}{0.65} &      \rcell{70.86}{0.67} &      \rcell{58.66}{0.48} \\
       & \osrcolor IForest \citeignore{iforest_detector} &                  \emptycell &      \rcell{55.87}{0.54} &      \rcell{55.44}{0.48} &      \rcell{52.23}{0.19} \\
       & \osrcolor OCVSM \citeignore{ocsvm_detector} &                  \emptycell &      \rcell{69.15}{0.67} &      \rcell{69.10}{0.69} &      \rcell{57.32}{0.45} \\
       & \osrcolor PCA \citeignore{pca_detector} &                  \emptycell &      \rcell{67.04}{0.67} &      \rcell{66.35}{0.69} &      \rcell{56.66}{0.38} \\
       & \osrcolor COPOD \citeignore{copod_detector} &                  \emptycell &      \rcell{50.26}{0.63} &      \rcell{51.77}{0.52} &      \rcell{50.77}{0.16} \\
       & \fslcolor SimpleShot \citeignore{wang2019simpleshot} &         \rcell{65.68}{0.62} &      \rcell{63.92}{0.58} &      \rcell{62.89}{0.54} &      \rcell{54.97}{0.29} \\
       & \fslcolor Baseline ++ \citeignore{Chen19} &         \rcell{65.68}{0.62} &      \rcell{64.61}{0.59} &      \rcell{63.41}{0.55} &      \rcell{55.38}{0.30} \\
       & \fslcolor FEAT \citeignore{ye2020few} &         \rcell{65.93}{0.63} &      \rcell{55.75}{0.42} &      \rcell{55.51}{0.39} &      \rcell{50.00}{0.00} \\
       & \fsosrcolor SnatcherF \citeignore{jeong2021few} &         \rcell{65.93}{0.63} &      \rcell{69.43}{0.63} &      \rcell{68.79}{0.64} &      \rcell{57.81}{0.42} \\
       & \fsosrcolor OpenMax \citeignore{bendale2016towards} &         \rcell{65.68}{0.62} &      \rcell{70.90}{0.66} &      \rcell{70.42}{0.69} &      \rcell{58.66}{0.48} \\
       & \fsosrcolor PROSER \citeignore{zhou2021learning} &         \rcell{65.04}{0.62} &      \rcell{31.43}{0.67} &      \rcell{39.99}{0.35} &      \rcell{48.49}{0.08} \\
       & \tfslcolor LaplacianShot \citeignore{ziko2020laplacian} &  \rcellsndbest{70.80}{0.72} &      \rcell{53.20}{0.79} &      \rcell{54.52}{0.61} &      \rcell{51.98}{0.24} \\
       & \tfslcolor BDCSPN \citeignore{liu2020prototype} &         \rcell{69.47}{0.70} &      \rcell{56.91}{0.69} &      \rcell{57.78}{0.58} &      \rcell{52.19}{0.26} \\
       & \tfslcolor TIM-GD \citeignore{boudiaf2020transductive} &         \rcell{69.28}{0.72} &      \rcell{55.73}{0.54} &      \rcell{55.49}{0.43} &      \rcell{52.25}{0.20} \\
       & \tfslcolor PT-MAP \citeignore{hu2021leveraging} &         \rcell{67.77}{0.66} &      \rcell{61.25}{0.57} &      \rcell{60.28}{0.51} &      \rcell{54.07}{0.27} \\
       & \tfsosrcolor OSTIM \citeignore{boudiaf2022ostim} &         \rcell{69.55}{0.69} &      \rcell{74.38}{0.61} &      \rcell{75.04}{0.64} &      \rcell{59.79}{0.48} \\
       & \ourscolor EOL (ours) &     \rcellbest{70.95}{0.75} &  \rcellbest{75.70}{0.67} &  \rcellbest{76.06}{0.69} &  \rcellbest{60.94}{0.61} \\
\midrule
\midrule
\sidecell{17}{5-shot} & \osrcolor \knn \citeignore{knn_detector} &                  \emptycell &      \rcell{77.36}{0.60} &      \rcell{77.61}{0.60} &      \rcell{62.20}{0.58} \\
       & \osrcolor  IForest \citeignore{iforest_detector} &                  \emptycell &      \rcell{63.61}{0.58} &      \rcell{62.30}{0.55} &      \rcell{55.14}{0.32} \\
       & \osrcolor OCVSM \citeignore{ocsvm_detector} &                  \emptycell &      \rcell{75.58}{0.58} &      \rcell{76.25}{0.60} &      \rcell{60.18}{0.50} \\
       & \osrcolor  PCA \citeignore{pca_detector} &                  \emptycell &      \rcell{75.72}{0.58} &      \rcell{75.85}{0.59} &      \rcell{60.96}{0.51} \\
       &  \osrcolor COPOD \citeignore{copod_detector} &                  \emptycell &      \rcell{52.68}{0.67} &      \rcell{53.53}{0.55} &      \rcell{51.59}{0.21} \\
       &  \fslcolor SimpleShot \citeignore{wang2019simpleshot} &         \rcell{81.18}{0.44} &      \rcell{70.84}{0.62} &      \rcell{70.17}{0.59} &      \rcell{58.06}{0.41} \\
       & \fslcolor Baseline ++ \citeignore{Chen19} &         \rcell{81.29}{0.43} &      \rcell{70.25}{0.54} &      \rcell{68.84}{0.53} &      \rcell{58.21}{0.34} \\
       & \fslcolor FEAT \citeignore{ye2020few} &         \rcell{81.09}{0.43} &      \rcell{58.55}{0.46} &      \rcell{58.71}{0.46} &      \rcell{50.00}{0.00} \\
       & \fsosrcolor SnatcherF \citeignore{jeong2021few} &         \rcell{81.09}{0.43} &      \rcell{77.70}{0.58} &      \rcell{77.48}{0.60} &      \rcell{62.71}{0.55} \\
     & \fsosrcolor  OpenMax \citeignore{bendale2016towards} &         \rcell{81.70}{0.43} &      \rcell{77.51}{0.57} &      \rcell{77.58}{0.59} &      \rcell{62.33}{0.55} \\
       & \fsosrcolor PROSER \citeignore{zhou2021learning} &         \rcell{81.27}{0.44} &      \rcell{62.38}{0.70} &      \rcell{62.80}{0.70} &      \rcell{54.59}{0.27} \\
    & \tfslcolor LaplacianShot \citeignore{ziko2020laplacian} &         \rcell{82.37}{0.45} &      \rcell{61.96}{0.79} &      \rcell{61.19}{0.67} &      \rcell{55.07}{0.35} \\
    & \tfslcolor BDCSPN \citeignore{liu2020prototype} &         \rcell{81.98}{0.45} &      \rcell{61.47}{0.73} &      \rcell{62.16}{0.64} &      \rcell{53.53}{0.32} \\
    & \tfslcolor  TIM-GD \citeignore{boudiaf2020transductive} &         \rcell{82.32}{0.43} &      \rcell{63.72}{0.58} &      \rcell{62.62}{0.52} &      \rcell{55.38}{0.28} \\
    & \tfslcolor  PT-MAP \citeignore{hu2021leveraging} &         \rcell{78.89}{0.47} &      \rcell{66.82}{0.61} &      \rcell{65.73}{0.57} &      \rcell{56.30}{0.37} \\
    & \tfsosrcolor OSTIM \citeignore{boudiaf2022ostim} &         \rcell{82.25}{0.43} &      \rcell{83.79}{0.43} &      \rcell{84.24}{0.45} &      \rcell{67.45}{0.59} \\ 
    & \ourscolor EOL (Ours) &     \rcellbest{83.72}{0.42} &  \rcellbest{85.88}{0.43} &  \rcellbest{86.02}{0.44} &  \rcellbest{70.60}{0.66} \\
\bottomrule
\end{tabular}
}
\end{table}
}
